NFR: Neural Feature-Guided Non-Rigid Shape Registration

In this paper, we propose a novel learning-based framework for 3D shape registration, which overcomes the challenges of significant non-rigid deformation and partiality undergoing among input shapes, and, remarkably, requires no correspondence annotation during training. Our key insight is to incorporate neural features learned by deep learning-based shape matching networks into an iterative, geometric shape registration pipeline. The advantage of our approach is two-fold -- On one hand, neural features provide more accurate and semantically meaningful correspondence estimation than spatial features (e.g., coordinates), which is critical in the presence of large non-rigid deformations; On the other hand, the correspondences are dynamically updated according to the intermediate registrations and filtered by consistency prior, which prominently robustify the overall pipeline. Empirical results show that, with as few as dozens of training shapes of limited variability, our pipeline achieves state-of-the-art results on several benchmarks of non-rigid point cloud matching and partial shape matching across varying settings, but also delivers high-quality correspondences between unseen challenging shape pairs that undergo both significant extrinsic and intrinsic deformations, in which case neither traditional registration methods nor intrinsic methods work. Our code is available at https://github.com/rqhuang88/NFR.

==> Figs/mit.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/mit.png}
    \caption{Qualitative showcase of different source shape selection. Though test it on the largest connected component of the input mesh, DPFM~\cite{attaiki2021dpfm}  falls short in performance .     }\label{fig:mit}
    % \vspace{-0.8em}
\end{figure}

==> Figs/realscan.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/realscan.png}
    \caption{ Qualitative results of noisy real scans. Our method transfer the facial details, strips in the T-shirt and arm precisely and smoothly}\label{fig:realscan}
    % \vspace{-0.8em}
\end{figure}

==> Figs/shrec07.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{Figs/shrec07.png}
    \caption{Qualitative comparison with HCLV2S~\cite{huang20} on matching heterogeneous partial point clouds.  }\label{fig:shrec07}
    % \vspace{-0.8em}
\end{figure}

==> Sec/abstract.tex <==
\begin{abstract}
In this paper, we propose a novel learning-based framework for 3D shape registration, which overcomes the challenges of significant non-rigid deformation and partiality undergoing among input shapes, and, remarkably, requires \emph{no} correspondence annotation during training. 
Our key insight is to incorporate neural features learned by deep learning-based shape matching networks into an iterative, geometric shape registration pipeline. 
The advantage of our approach is two-fold -- On one hand, neural features provide more accurate and semantically meaningful correspondence estimation than spatial features (\emph{e.g., } coordinates), which is critical in the presence of large non-rigid deformations; On the other hand, the correspondences are dynamically updated according to the intermediate registrations and filtered by consistency prior, which prominently robustify the overall pipeline.
Empirical results show that, with as few as dozens of training shapes of limited variability, our pipeline achieves state-of-the-art results on several benchmarks of non-rigid point cloud matching and partial shape matching across varying settings, but also delivers high-quality correspondences between unseen challenging shape pairs that undergo both significant extrinsic and intrinsic deformations, in which case neither traditional registration methods nor intrinsic methods work. 




% In this paper, we propose a novel learning-based framework for non-rigid shape registration \emph{without correspondence supervision}, which can tackle the problem of \emph{partial} shape matching as well. Namely, we deform source mesh towards the target point cloud, guided by correspondences induced by high-dimensional embeddings learned from deep functional maps (DFM). In particular, the correspondences are dynamically updated according to the intermediate registrations and filtered by consistency prior, which prominently robustify the overall pipeline. In addition, we distinctively robustify partial functional maps with a novel scheme, which computes partial shapes' spectral embeddings conditioned on their full version, so as to solve the \emph{partial-2-full} registration problem. Specifically, equipped with the robustified partial functional maps, we train a point feature extractor on a set of complete meshes in a self-supervised manner. Empirical results show that, with as few as dozens of training shapes of limited variability, our pipeline achieves state-of-the-art results on several benchmarks of non-rigid point cloud matching and partial shape matching across varying settings, but also delivers high-quality correspondences between unseen challenging shape pairs that undergo both significant extrinsic and intrinsic deformations, in which case neither traditional registration methods nor intrinsic methods work. 
 % The code is available at \url{https://github.com/rqhuang88/DFR}.
\end{abstract}
\begin{IEEEkeywords}
Shape Registration, Deep Functional Maps, Non-rigid Shape Matching
\end{IEEEkeywords}
